Nonlinear Acceleration of Momentum and Primal-Dual Algorithms

We describe convergence acceleration schemes for multistep optimization algorithms. The extrapolated solution is written as a nonlinear average of the iterates produced by the original optimization method. Our analysis does not need the underlying fixed-point operator to be symmetric, hence handles e.g. algorithms with momentum terms such as Nesterov's accelerated method, or primal-dual methods. The weights are computed via a simple linear system and we analyze performance in both online and offline modes. We use Crouzeix's conjecture to show that acceleration performance is controlled by the solution of a Chebyshev problem on the numerical range of a non-symmetric operator modeling the behavior of iterates near the optimum. Numerical experiments are detailed on logistic regression problems.

==> Numerical_Experiments.tex <==
\section{Numerical Results}\label{s:numres}
We now study the performance of our techniques on several classical applications: image processing problems using extrapolation on Chambolle-Pock's algorithm and $\ell_2$-regularized logistic regression using acceleration on Nesterov's accelerated method\footnote{The source code for the numerical experiments can be found on GitHub at \url{https://github.com/windows7lover/RegularizedNonlinearAcceleration}}. We also study acceleration on stochastic gradient algorithms with momentum terms used for training neural networks. 

\subsection{Accelerating Algorithms with Momentum Terms}
The following numerical experiments seek to highlight the benefits of RNA in its offline and online versions when applied to the gradient method (with or without momentum term). Since the complexity grows quadratically with the number $N$ of points in the sequences $\{x_i\}$ and $\{y_i\}$, we will use RNA with a fixed window size ($N=5$ for stochastic and $N=10$ for convex problems) and regularization parameter $\lambda=10^{-8}\|R^TR\|_2$ in all these experiments. These values are sufficiently large to show a significant improvement in the rate of convergence, but can of course be fine-tuned. 

\FloatBarrier
\subsubsection{Logistic Regression}

We solve a classical regression problem on the Madelon-UCI dataset \citep{guyon2003design} using the logistic loss with $\ell_2$ regularization. The regularization has been set such that the condition number of the function is equal to $10^{6}$. We compare to standard algorithms such as the simple gradient scheme, Nesterov's method for smooth and strongly convex objectives \citep{nesterov2013introductory} and L-BFGS. For the step length parameter, we used a backtracking line-search strategy. We compare these methods with their offline RNA accelerated counterparts, as well as with the online version of RNA described in~\eqref{eq:algo_rna}. 

\begin{figure}[h!t]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/offline_madelon.eps}
    \includegraphics[width=0.47\textwidth]{figs/online_madelon.eps}
    \caption{Logistic loss on the Madelon \citep{guyon2003design}. Comparison between offline (\textit{left}) and online (\textit{right}) strategies for RNA on gradient and Nesterov's method. We use $\ell$-BFGS (with $\ell=100$ gradients stored in memory) as baseline. Clearly, one step of acceleration improves the accuracy. The performance of online RNA, which applies the extrapolation at \textit{each} step, is similar to that of L-BFGS methods, though RNA does not use line-search and requires 10 times less memory.}
    \label{fig:madelon}
\end{figure}
We observe in Figure \ref{fig:madelon} that offline RNA improves the convergence speed of gradient descent and Nesterov's method. However, the improvement is only a constant factor: the curves are shifted but have the same slope. Meanwhile, the online version greatly improves the rate of convergence, transforming the basic gradient method into an optimal algorithm competitive with line-search L-BFGS.

In contrast to most quasi-Newton methods (such as L-BFGS), RNA does \textit{not} require a Wolfe line-search to be convergent. This is because the algorithm is stabilized with a Tikhonov regularization. In addition, the regularization in a way controls the impact of the noise in the iterates, making the RNA algorithm suitable for stochastic iterations \citep{scieur2017nonlinear}.

\FloatBarrier
\begin{comment}

\subsubsection{Training CNNs for image classification.} Because one stochastic iteration is not informative due to the noise, we refer to $x_k$ as the model parameters (including batch normalization statistics) corresponding to the final iteration of the epoch $k$. In this case, we do not have an explicit access to ``$(x_k-y_{k-1})$'', so we will estimate it during the stochastic steps.  Let $y_{k}^{(t)}$ be the parameters of the network at epoch $k$ after $t$ stochastic iterations, and $x_k^{(t+1)}$ be the parameters after one stochastic gradient step. Then, for a data set of size $D$,
\[
    x_{k}-y_{k-1} \approx \frac{1}{D} \sum_{t=1}^D (x_k^{(t+1)}-y_k^{(t)}) = -h\frac{1}{D} \sum_{t=1}^D \nabla f(y_{k}^{(t)}).
\]
This means the matrix $R$ in Algorithm \ref{algo:block-rna} will be the matrix of (estimated) gradients. Because the learning curve is highly dependent on the learning rate schedule, we decided to use a linearly decaying learning rate to better illustrate the benefits of acceleration, even if acceleration also works with a constant learning rate schedule (see \citep{scieur2018nonlinear} and Figure \ref{fig:proto}). In all our experiments, until epoch~$T$, the learning rate decreases linearly from an initial value $h_0$ to a final value $h_T$, with
\BEQ
    h_k = h_0+(k/T)(h_T-h_0). \label{eq:lr_gen}
\EEQ
We then continue the optimization during $10$ additional epochs using $h_T$ to stabilize the curve. We summarize the parameters used for the optimization in Table \ref{tab:parameters}.
{
\begin{table}[h!t]
	\renewcommand{\arraystretch}{1.2}
    \centering
    \begin{tabular}{l|ccc}
                         & $h_0$ & $h_T$ & momentum \\
        \hline
        SGD and Online RNA \eqref{eq:algo_rna}   & 1.0   & 0.01   & 0  \\  
        SGD + momentum                             & 0.1   & 0.001  & 0.9\\ 
    \end{tabular}
    \caption{Parameters used in \eqref{eq:lr_gen} to generate the learning rate for optimizers. We used the same setting for their accelerated version with RNA.}
    \label{tab:parameters}
\end{table}
}
    
\FloatBarrier
\subsubsection{CIFAR10}
CIFAR-10 is a standard 10-class image dataset comprising $5 \cdot 10^4$ training samples and $10^4$ samples for testing. Except for the linear learning rate schedule above, we follow the standard practice for CIFAR-10. We applied the standard augmentation via padding of $4$ pixels. We trained the networks VGG19, ResNet-18 and DenseNet121 during $100$ epochs ($T = 90$) with a weight decay of $5\cdot10^{-4}$.

We observe in Figure~\ref{fig:cifar10_online} that the online version does not perform as well as in the convex case. More surprisingly, it is outperformed by its offline version (Figure~\ref{fig:cifar10_offline}) which computes the iterates on the side. In fact, the offline experiments detailed in~Figure~\ref{fig:cifar10_offline} exhibit much more significant gains. It produces a similar test accuracy, and the offline version converges faster than SGD, especially for early iterations. We reported speedup factors to reach a certain tolerance in Table \ref{tab:speedup}. This suggests that the offline version of RNA is a good candidate for training neural networks, as it converges faster while guaranteeing performance \textit{at least} as good as the reference algorithm.



\begin{figure}[h!t]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/proto_large.eps}
    \includegraphics[width=0.47\textwidth]{figs/proto_zoom.eps}
    \caption{Prototyping networks: acceleration (bottom curves) gives a smoother convergence, producing a clearer ranking of architectures, much earlier (we use a flat learning rate). The right plot zooms on left one.}
    \label{fig:proto}
\end{figure}

\begin{figure}[h!t]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/loss_offline_rna_cifar_vgg.eps}
    \includegraphics[width=0.47\textwidth]{figs/error_offline_rna_cifar_vgg.eps}
    \includegraphics[width=0.47\textwidth]{figs/loss_offline_rna_cifar.eps}
    \includegraphics[width=0.47\textwidth]{figs/error_offline_rna_cifar.eps}
    \includegraphics[width=0.47\textwidth]{figs/loss_offline_rna_cifar_densenet.eps}
    \includegraphics[width=0.47\textwidth]{figs/error_offline_rna_cifar_densenet.eps}
    \caption{(Top to bottom) VGG, Resnet-18 and Densenet networks on Cifar10, 100 epochs. SGD with and without momentum, and their off-line accelerated versions with a window size $5$. Left: training loss. Right: top-1 validation error.}
    \label{fig:cifar10_offline}
\end{figure}

\begin{figure}[h!t]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/loss_orna_cifar.eps}
    \includegraphics[width=0.47\textwidth]{figs/error_orna_cifar.eps}
    \caption{Online RNA for training a Resnet-18 on CIFAR-10.}
    \label{fig:cifar10_online}
\end{figure}




\begin{table}[h!t]
	\centering
	\renewcommand{\arraystretch}{1.2}
	\begin{tabular}{c|cccc}
		Tolerance & SGD & SGD+momentum & SGD+RNA & SGD+momentum+RNA \\
		\hline
		5.0\% & 68 (0.87$\times$)  &  59  &  21 (2.81$\times$)  &  \textbf{16} (3.69$\times$) \\
		2.0\% & 78 (0.99$\times$)  &  77  &  47 (1.64$\times$)  &  \textbf{40} (1.93$\times$) \\
		1.0\% & 82 (1.00$\times$)  &  82  &  67 (1.22$\times$)  &  \textbf{59} (1.39$\times$) \\
		0.5\% & 84 (1.02$\times$)  &  86  &  75 (1.15$\times$)  &  \textbf{63} (1.37$\times$) \\
		0.2\% & 86 (1.13$\times$)  &  97  &  \textbf{84} (1.15$\times$)  &  85 (1.14$\times$) \\
	\end{tabular}
	\begin{tabular}{c|cccc}
		Tolerance & SGD & SGD+momentum & SGD+RNA & SGD+momentum+RNA \\
		\hline
		5.0\% & 69 ($0.87\times$)  &  60  &  26 ($2.31\times$)  &  \textbf{24} ($2.50\times$) \\
		2.0\% & 83 ($0.99\times$)  &  82  &  52 ($1.58\times$)  &  \textbf{45} ($1.82\times$) \\
		1.0\% & 84 ($1.02\times$)  &  86  &  71 ($1.21\times$)  &  \textbf{60} ($1.43\times$) \\
		0.5\% & 89 ($0.98\times$)  &  87  &  73 ($1.19\times$)  &  \textbf{62} ($1.40\times$) \\
		0.2\% & \textbf{N/A} &  90  &  99 ($0.90\times$)  &  \textbf{63} ($1.43\times$) \\
	\end{tabular}
	\begin{tabular}{c|cccc}
		Tolerance & SGD & SGD+momentum & SGD+RNA & SGD+momentum+RNA \\
		\hline
		5.0\% & 65 (0.86$\times$)  &  56  &  22 (2.55$\times$)  &  \textbf{13} (4.31$\times$) \\
		2.0\% & 80 (0.98$\times$)  &  78  &  45 (1.73$\times$)  &  \textbf{38} (2.05$\times$) \\
		1.0\% & 83 (1.00$\times$)  &  83  &  60 (1.38$\times$)  &  \textbf{56} (1.48$\times$) \\
		0.5\% & 87 (0.99$\times$)  &  86  &  80 (1.08$\times$)  &  \textbf{66} (1.30$\times$) \\
		0.2\% & 92 (1.01$\times$)  &  93  &  86 (1.08$\times$)  &  \textbf{75} (1.24$\times$) \\
	\end{tabular}
	\caption{Number of epochs required to reach the best test accuracy +$\text{\textit{ Tolerance}}\%$ on CIFAR10 with a (\textit{top} to \textit{bottom}) VGG, Resnet18 and Densenet, using several algorithms. The best accuracies are $6.54\%$ (VGG), $5.0\%$ (Resnet-18) and $4.62\%$(Densenet). The speed-up compared to the SGD+momentum baseline is in parenthesis.}
    \label{tab:speedup}
\end{table}

% \FloatBarrier

\subsubsection{ImageNet}
Here, we apply the RNA algorithm to the standard ImageNet dataset. We trained the networks during $90$ epochs ($T = 80$) with a weight decay of $10^{-4}$. We reported the test accuracy on Figure \ref{fig:imnet} for the networks ResNet-50 and ResNet-152. We only tested the offline version of RNA here, because in previous experiments it gives better result than its online counterpart.

We again observe that the offline version of Algorithm \ref{algo:block-rna} improves the convergence speed of SGD with and without momentum. In addition, we show a substantial improvement of the accuracy over the non-accelerated baseline. The improvement in the accuracy is reported in Table~\ref{tab:accuracy}. Interestingly, the resulting training loss is smoother than its non accelerated counterpart, which indicates a noise reduction.


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/imnet_resnet50.eps}
    \includegraphics[width=0.47\textwidth]{figs/imnet_resnet152.eps}
    \caption{Training a Resnet-52 (\textit{left}) and ResNet-152 (\textit{right}) on validation ImageNet for 90 epochs using SGD with and without momentum, and their off-line accelerated versions.}
    \label{fig:imnet}
\end{figure}

\begin{table}[ht]
	\centering
	\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|ccccc}
	~& Pytorch & SGD & SGD+mom. & SGD+RNA & SGD+mom.+RNA \\
	\hline
	Resnet-50 & 23.85 & 23.808 & 23.346 & 23.412 (-0.396\%) & \textbf{22.914} (-0.432\%) \\
	Resnet-152 & 21.69 & N/A & 21.294 & N/A & \textbf{20.884} (-0.410\%) \\
\end{tabular}
\caption{Best validation top-1 error percentage on ImageNet. In parenthesis the improvement due to RNA. The first column corresponds to the performance of Pytorch pre-trained models.}
\label{tab:accuracy}
\end{table}

\end{comment}
%\FloatBarrier

\subsection{Algorithms with Non-symmetric Operators}
We conducted numerical experiments to illustrate the performance of RNA on non-symmetric algorithms. We consider two different classes of problems: smooth strongly convex problems and non-smooth convex problems.

\subsubsection{Smooth Problems}
We consider ridge regression and $l_2$ regularized logistic regression problems which are of the form,
\begin{equation*}
    h(x) : = f(Ax) + g(x)
\end{equation*}
where $f(Ax) = \frac{1}{2}\|Ax - b\|^2$ for ridge regression and $f(Ax) = \sum \log(1 + \exp(- a_i^Txb_i))$ for logistic regression, and $g(x) = \frac{\mu}{2}\|x\|^2$. The following methods are tested in this experiment. % We use the datasets listed in Table \ref{?} with different regularization constants $\mu$.
\begin{itemize}
    \item \textbf{GD.} The gradient descent method $x_{k+1} = x_k - \frac{1}{L}\nabla h(x_k)$, where $L$ is the Lipschitz constant of the gradient. 
    \item \textbf{Nesterov.} The Nesterov's accelerated gradient method \citep{nesterov2013introductory}
    \begin{equation*}
    \begin{aligned}
    x_{k+1} &= y_k - \frac{1}{L}\nabla h(y_k) \qquad
    y_{k+1} &= y_k + \beta(y_k - y_{k-1})
    \end{aligned}
    \end{equation*}
    where $\beta = \frac{\sqrt{L} - \sqrt{\mu}}{\sqrt{L} + \sqrt{\mu}}$, $L$ is the Lipschitz constant of the gradient. 
    \item \textbf{L-BFGS.} The L-BFGS method  \citep{liu1989limited} $x_{k+1} = x_k - \alpha_kH_k\nabla h(x_k)$ where the steplength parameter $\alpha_k$ is chosen via Armijo backtracking line search and the memory parameter is chosen to be $10$.
    \item \textbf{PDGM.} The primal-dual gradient method \citep{chambolle2011first,arrowhurwicz1960}
    \begin{equation*}
    \begin{aligned}
        y_{k+1} &= Prox_{f^*}^{\sigma}(y_k + \sigma Ax_k) \qquad
        x_{k+1} &= Prox_g^{\tau}(x_k - \tau A^*y_{k+1})
    \end{aligned}
    \end{equation*}
    where $\sigma = \frac{1}{\|A\|}\sqrt{\frac{\mu}{\delta}}$, $\tau = \frac{1}{\|A\|}\sqrt{\frac{\delta}{\mu}}$, $\delta$ is the strong convexity parameters of $f^*$. 
    \item \textbf{PDGM + Momentum.} The primal-dual gradient method with momentum \citep{chambolle2011first}
    \begin{equation*}
    \begin{aligned}
        y_{k+1} = Prox_{f^*}^{\sigma}(y_k + \sigma A\bar{x}_k)& \quad
        x_{k+1} = Prox_g^{\tau}(x_k - \tau A^*y_{k+1}) \\
        \bar{x}_{k+1} &= x_{k+1} + \theta (x_{k+1} - x_{k}) 
    \end{aligned}
    \end{equation*}
    where $\sigma = \frac{1}{\|A\|}\sqrt{\frac{\mu}{\delta}}$, $\tau = \frac{1}{\|A\|}\sqrt{\frac{\delta}{\mu}}$, $\theta = \frac{1}{1 + \frac{2\sqrt{\mu\delta}}{\|A\|}}$, $\delta$ is the strong convexity parameters of $f^*$. 
    
\end{itemize}

The Lipschitz constant $L$ is $\|A\|^2 + \mu$ for ridge regression and is $\frac{\|A\|^2}{4} + \mu$ for logistic regression. The strong convexity parameter $\delta$ of the dual function $f^*$ is $1$ for ridge regression and is $4$ for logistic regression.   The proximal operators used in the primal - dual algorithms have closed form solutions for ridge regression. That is, $Prox_{g}^\tau(x) = \frac{1}{1 + \tau\mu}$ and $Prox_{f^*}^\sigma(y) =\frac{y - \sigma b}{1 + \sigma}$. In logistic regression, the approximate proximal operator of $f^*$ is obtained by running Newton's method till some tolerance on the accuracy is achieved or a maximum of $100$ iterations is reached. Note that the dominant cost in computing the gradients or proximal operators is the cost of computing the matrix vector products $Ax$ and $A^*y$ which are of the order $O(Nd)$ and the cost of performing Newton's method to obtain the proximal operator is of order $N$ times the maximum number of iterations $t$. Therefore, when $t < d$ one can ignore the additional cost of performing Newton's method.       

We use online RNA on GD, Nesterov and PDGM with a fixed window size $m = 10$ and set $\lambda = 10^{-8}\|R^TR\|_2$.  As discussed in Section \ref{s:algos}, RNA can be applied only with specific choices of the step-length parameters in the case of primal-dual methods. In the case of smooth problems, we observe that the choice $\tau = \frac{1}{\|A\|}$ and $\sigma=\frac{1}{\|A\|}$ yields stability for applying RNA on PDGM. We note this choice is not an optimal choice and one can improve the results by suitably tuning these parameters. 

Figure \ref{fig:madelon_nonsym_quad1} shows the performance of different variants of the primal-dual algorithms on ridge regression problems for two different regularization constants. We observe that there is no significant difference in the performance of the method with the momentum term $(\theta)$ as compared to the one with no momentum term. We also observe that although the choice of the steplength parameters mentioned above have consistent performance across different problems, the improvements obtained with RNA are not very significant. However, choosing $\sigma = \tau = 1/\|A\|$ and applying RNA to the PDGM has consistently outperformed all other variants. This is in consistent with theoretical observations made in Section \ref{s:algos} that one can find optimal steplength parameters for which RNA is stable and obtains the optimal performance. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/MadelonNormalized_quadratic_100e-02_PrimalLoss1.eps}
    \includegraphics[width=0.47\textwidth]{figs/MadelonNormalized_quadratic_100e+02_PrimalLoss1.eps}
    \caption{Quadratic loss on the Madelon \citep{guyon2003design}. Left : $\mu = 10^{-2}$. Right : $\mu = 10^{2}$. Comparison of online RNA with other variants of primal-dual gradient methods. }
    \label{fig:madelon_nonsym_quad1}
\end{figure}

Figure \ref{fig:madelon_nonsym_quad2} compares the performance of primal-dual algorithms with other well know algorithms on ridge regression problems. We observe that Nesterov's accelerated gradient method and primal-dual gradient method consistently outperformed gradient descent as suggested by the theory as these methods achieve the optimal rates. The RNA variants of gradient descent and primal-dual methods are competitive and outperform their base algorithms. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/MadelonNormalized_quadratic_100e-02_PrimalLoss3.eps}
    \includegraphics[width=0.47\textwidth]{figs/MadelonNormalized_quadratic_100e+02_PrimalLoss3.eps}
    \caption{Quadratic loss on the Madelon \citep{guyon2003design}. Left : $\mu = 10^{-2}$. Right : $\mu = 10^{2}$. Comparison of online RNA on primal-dual gradient methods with other first-order algorithms.}
    \label{fig:madelon_nonsym_quad2}
\end{figure}

Figure \ref{fig:madelon_nonsym_logistic1} shows the performance of the methods on logistic regression problems. We observe that the RNA variants have substantially improved the performance of the base algorithms. The L-BFGS method with Armijo backtracking line-search has the optimal performance across different problems and the RNA variants are competitive to this method.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/MadelonNormalized_logistic_100e-02_PrimalLoss2.eps}
    \includegraphics[width=0.47\textwidth]{figs/MadelonNormalized_logistic_100e+02_PrimalLoss2.eps}
    \caption{Logistic loss on the Madelon \citep{guyon2003design}. Left : $\mu = 10^{-2}$. Right : $\mu = 10^{2}$. Comparison of online RNA on primal-dual gradient methods with other first-order algorithms.}
    \label{fig:madelon_nonsym_logistic1}
\end{figure}


We now illustrate the effects of RNA on Nesterov's accelerated gradient method. As discussed in Section~\ref{s:algos}, RNA is applied to sequence of iterates that are obtained after regular intervals, and the length of the interval needs to be chosen based on the problem characteristics. Figures \ref{fig:madelon_nonsym_quad_nest} and \ref{fig:madelon_nonsym_logistic_nest} compare the performance of RNA on Nesterov's sequence of iterates for various interval lengths $p$. We observe that the length of the interval has significant effect on the performance of the algorithm and this choice depends on the trade off between stability and speed of convergence. That is, the larger the interval length, higher the chance of getting an accelerated sequence but lower the speed of convergence. Higher powers are generally needed for highly ill-conditioned problems. Due to these difficulties, it is clear that for simple momentum terms, one should consider the symmetric part of these iterations and apply RNA on these sequences as discussed in Section \ref{s:momentum}. We report the results with this approach in the next section.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/MadelonNormalized_quadratic_100e-02_PrimalLoss_Nest.eps}
    \includegraphics[width=0.47\textwidth]{figs/MadelonNormalized_quadratic_100e+02_PrimalLoss_Nest.eps}
    \caption{Quadratic loss on the Madelon \citep{guyon2003design}. Left : $\mu = 10^{-2}$. Right : $\mu = 10^{2}$. Comparison of online RNA on different iterate sampling rates, i.e. different powers of the operator for  Nesterov's strongly convex acceleration algorithm.}
    \label{fig:madelon_nonsym_quad_nest}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/MadelonNormalized_logistic_100e-02_PrimalLoss_Nest.eps}
    \includegraphics[width=0.47\textwidth]{figs/MadelonNormalized_logistic_100e+02_PrimalLoss_Nest.eps}
    \caption{Logistic loss on Madelon \citep{guyon2003design}. Left : $\mu = 10^{-2}$. Right : $\mu = 10^{2}$. Comparison of online RNA on different iterate sampling rates, i.e. different powers of the operator for  Nesterov's strongly convex acceleration algorithm.}
    \label{fig:madelon_nonsym_logistic_nest}
\end{figure}

Lastly, we compare the performance of offline, restart and online versions of RNA on primal-dual gradient methods in Figure \ref{fig:madelon_nonsym_logistic_offline}. We observe that the improvement in the performance is more pronounced in the online version of RNA as compared to the offline version.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/MadelonNormalized_logistic_100e-02_PrimalLoss_Offline.eps}
    \includegraphics[width=0.47\textwidth]{figs/MadelonNormalized_logistic_100e+02_PrimalLoss_Offline.eps}
    \caption{Logistic loss on the Madelon \citep{guyon2003design}. Left : $\mu = 10^{-2}$. Right : $\mu = 10^{2}$. Comparison of offline, restart and online variants of RNA on primal-dual gradient methods. }
    \label{fig:madelon_nonsym_logistic_offline}
\end{figure}


\subsubsection{Non-Smooth Problems}
We consider denoising an image that is degraded by Gaussian noise using total variation. We refer the reader to \cite{chambolle2016introduction} for details about the total variation models. The optimization problem is given as, 

\begin{equation*}
    \min_{x} \|\nabla x\|_1 + \frac{\mu}{2}\|x - b\|^2
\end{equation*}
where,
\begin{equation*}
    \|\nabla x\|_1 = \sum_{i,j} |(\nabla x)_{i,j}| \qquad |(\nabla x)_{i,j}| = \sqrt{((\nabla x)_{i,j}^1)^2 + ((\nabla x)_{i,j}^2)^2}
\end{equation*}
and $b$ is a $256$ by $256$ noisy input image. This optimization problem is in the form \eqref{prob:primal} with $f(\nabla x) = \|\nabla x\|_1$ and $g(x) = \frac{\mu}{2}\|x - b\|^2$. 
The gradient operator $\nabla x$ is discretized by forward differencing (see \cite{chambolle2011first}). The convex conjugate of $f$ is an indicator function of the convex set $P$ where,
\begin{equation*}
    P =\{p: \|p\|_{\infty} \leq 1\},  \qquad |p\|_{\infty} = \max_{i,j}|p_{i,j}|,  \qquad |p_{i,j}| = \sqrt{(p_{i,j}^1)^2 + (p_{i,j}^2)^2}
\end{equation*}
and so the proximal operator is a point wise projection on to this set. That is $Prox_{f^*}^{\sigma}(p)_{i,j} =\frac{p_{i,j}}{\max(1,|p_{i,j}|)}$.

We compare the performance of the two variants of primal-dual methods with RNA for two different noise levels $\zeta$ with two different regularization constants $\mu$. The step-length parameters are chosen adaptively at each iteration as follows:
\begin{itemize}
    \item \textbf{PDGM}
    \begin{equation*}
        \hat{\theta}_{k} = \frac{1}{\sqrt{1 + 2\gamma\tau_k}}\qquad\sigma_{k+1} = \frac{\sigma_k}{\hat{\theta}_k} \qquad \tau_{k+1} = \tau
_{k}\hat{\theta}_k
    \end{equation*}
    with $\gamma = 0.2 \mu$, $\theta = 0$, $\tau_0 = 0.02$, $\sigma_0 = \frac{4}{\tau_0\|\nabla\|^2}$
    \item \textbf{PDGM + Momentum}
    \begin{equation*}
        \theta_{k} = \frac{1}{\sqrt{1 + 2\gamma\tau_k}}\qquad\sigma_{k+1} = \frac{\sigma_k}{\theta_k} \qquad \tau_{k+1} = \tau
_{k}\theta_k
    \end{equation*}
    with $\gamma = 0.7 \mu$ and $\sigma_0 = \tau_0 = \frac{1}{\|\nabla\|}$
\end{itemize}
with $\|\nabla \|^2 = 8$. These adaptive choices are the standard choices used in the literature and yield the optimal theoretical convergence rates for the momentum variants. We note that these parameters are not carefully fine-tuned to give the best performance for each variant but are chosen based on some simple observations. We used the offline RNA instead of online RNA as we consistently observed that the offline RNA is more robust in the high accuracy regime and the online variants needed some stability inducing techniques like linesearches. Moreover, for the online RNA, the improvement in the performance on these non-smooth problems is small and so the additional cost of solving the linear system is not well justified. 

\begin{figure}[h!t]
    \centering
    \includegraphics[width=0.2\textwidth]{figs/lena_noise01_tvl2_TrueImage.eps}\quad
    \includegraphics[width=0.2\textwidth]{figs/lena_noise01_tvl2_NoisyImage.eps}\quad
    \includegraphics[width=0.2\textwidth]{figs/lena_noise005_tvl2_NoisyImage.eps}
    \caption{Images used in the experiments. Left: True data. Middle: Noisy data with Gaussian noise $\zeta = 0.1$. Right: Noisy data with Gaussian noise $\zeta =0.05$}
    \label{fig:lenaimage}
\end{figure}

Table \ref{tab:imgdenoise} reports the number of iterations required for the distance between the primal function value and the optimal primal function value to be below certain accuracy. We observe that the PDGM + RNA has consistently outperformed the PDGM and its' momentum variant for all the accuracies.

\begin{table}[h!t]
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|ccc|ccc}
    & \multicolumn{3}{c|}{$\zeta = 0.1, \mu = 8$} & \multicolumn{3}{c}{$\zeta = 0.05, \mu = 16$}\\
	& $\epsilon=10^{-2}$ & $\epsilon=10^{-4}$ & $\epsilon=10^{-6}$ & $\epsilon=10^{-2}$ & $\epsilon=10^{-4}$ & $\epsilon=10^{-6}$ \\
	\hline
	PDGM & 488 &  1842  &  7146  &  257 &  943  &  3706 \\
	PDGM + Momentum & 377 &  1744  &  6813  &  226 &  921  &  3879 \\
	PDGM + offlineRNA & \textbf{221} &  \textbf{1151}  &  \textbf{5801}  &  \textbf{141} &  \textbf{671}  &  \textbf{3241} \\
\end{tabular}
\caption{Number of iterations required for the primal accuracy to be below $\epsilon$ on the images shown in Figure \ref{fig:lenaimage} using primal-dual gradient methods.}
\label{tab:imgdenoise}
\end{table}

==> contribution.tex <==
 % Another contribution is the convergence analysis in the case where $J_g$ is not symmetric anymore. This case happens usually when using \textit{primal-dual} methods, such as Chambolle-Pock \citep{chambolle2011first} algorithm.

==> link_polynomial.tex <==
We now link the accuracy of the extrapolation $\sum_{i=1}^k c_i y_{i-1}$ with the norm of a matrix polynomial $p(A)$, where $A$ is the linear fixed point operator in~\eqref{eq:lfpi}, under mild assumptions on the coefficients $\alpha^{(i)}_j$ and $\beta^{(i)}_j$ in \eqref{eq:iter}. 
%For simplicity, we analyze a combination of $y_{i-1}$, but in practice using the combination of $x_i$ is better since, for linear $g$, we have
For simplicity, we analyze the combination of $y_{i-1}$, but, in practice, it is better to use the combination of $x_i$ since, for linear $g$, we have
\[
    \sum_{i=1}^k c_i x_{i} = \sum_{i=1}^k c_i g(y_{i-1}) = g\left( \sum_{i=1}^k c_i y_{i-1} \right).
\]
so the points $x_i$ are one iteration ahead of $y_i$. We will prove
\BEA
    \min_{c : c^T\textbf{1} = 1} \left\|\sum_{i=1}^k c_i r_i\right\| &=& \min_{p\in \mathcal{P}_{k-1} : p(1) = 1} \|p(A)r_1\|\\ 
    & \leq & \|r_1\| \min_{p\in \mathcal{P}_{k-1} : p(1) = 1} \|p(A)\|, \label{eq:equality_combination_polynomial}
\EEA
where $\mathcal{P}_k$ is the linear space of polynomials of degree at most $k$. This then directly yields a convergence bound on $\|\sum_{i=0}^k c_i y_i-x^*\|$, since
\[
    \left\|\sum_{i=1}^k c_i y_{i-1}-x^*\right\| = \left\| (A-I)^{-1} \sum_{i=1}^k c_i (x_{i}-y_{i-1})\right\| \leq \left\|(A-I)^{-1}\right\| \left\|\sum_{i=1}^k c_i r_i\right\|.
\]
Thus, if the coefficients $c^*$ in \eqref{eq:cstar} are used, and if we assume $A-I$ invertible,
\BEQ \label{eq:bound_proximity_xstar}
    \left\|\sum_{i=1}^k c^*_i y_{i-1}-x^*\right\| \leq \left\|(A-I)^{-1}\right\|  \|r_1\| \min_{p\in \mathcal{P}_{k-1} : p(1) = 1} \|p(A)\|.
\EEQ
Studying nonlinear acceleration accuracy thus reduces to studying Chebyshev polynomials under constraint, and we now prove \eqref{eq:equality_combination_polynomial}.
\begin{theorem} \label{thm:convergence_rate_online_rna}
	Let $\{x_1,\, \ldots,\, x_k\}$ and $\{y_0,\, \ldots,\, y_{k-1}\}$ be the two sequences produced by running $k$ iterations of the optimization algorithm \eqref{eq:iter}, where
	$g(x)$ is the linear mapping \eqref{eq:lfpi} and $\alpha_i^{(k)}$, $\beta_i^{(k)}$ are arbitrary coefficients such that
	\[
		\alpha_N^{(k)} \neq 0 \quad \text{ and } \quad {\textstyle \sum_{i=1}^k} \alpha_i^{(k)} + {\textstyle \sum_{i=1}^{k}}  \beta_i^{(k)} = 1.
	\]
	Then,
	\BEQ\label{eq:equality_combination_polynomial_thm}
	    \min_{c : c^T\textbf{1} = 1} \left\|\sum_{i=1}^k c_i r_i\right\| = \min_{p\in \mathcal{P}_k : p(1) = 1} \|p(A)r_1\|. 
	\EEQ
	By \eqref{eq:bound_proximity_xstar}, extrapolation accuracy is then bounded by
	\[
        \left\|\sum_{i=1}^k c^*_i y_{i-1}-x^*\right\| \leq \left\|(A-I)^{-1}\right\|\|r_1\|\min_{p\in \mathcal{P}_{k-1} : p(1) = 1} \|p(A)\|.
    \]
\end{theorem}
\begin{proof}
For clarity, we remove the superscript $(k)$ on the parameters $\alpha$ and $\beta$, in the scope of this proof. The key part of the proof is showing the following relation,
\BEQ
    r_i = q_i(A)r_1, \label{eq:polynomial_r}
\EEQ
where $q_i$ is a polynomial of degree \textit{exactly} $i-1$, with $q_i(1)=1$. The rest of the proof is easy, since $\{r_i\}_{i=1\ldots k}$ are formed using independent polynomials (they all have different degrees). Since we have an independent family with $k$ elements, and the maximum degree of those polynomials is $k-1$ (which is $q_k$, associated to $r_k$), then we have a basis for $\mathcal{P}_{k-1}$. This means
\[
    \forall\, p \in \mathcal{P}_{k-1}, \quad \exists\, c \in \mathbb{R}^{k}: \sum_{i=1}^k c_i r_i = p(A)r_1.
\]
In addition, if we force $\sum_{i=1}^k c_i = 1$, then the coefficients of the resulting polynomial also sum to one since
\[
    p(1) = \sum_{i=1}^k c_i q_i(1) = \sum_{i=1}^k c_i = 1.
\]
This finally proves \eqref{eq:equality_combination_polynomial_thm}. It thus remains to show \eqref{eq:polynomial_r}. We will prove the claim by recursion. We start with the simple case $i=1$, i.e.,
\[
	r_1 = I r_1
\]
and the identity matrix $I$ indeed corresponds to the ``polynomial'' $p(A) = 1\cdot A^0$ of degree $0$, whose ``coefficients sum to one''. Now, assume the claim is true for $r_{i-1}$, and we will show it is also true for $r_{i}$. Indeed,
\BEA
	r_{i} & = & x_{i} - y_{i-1}, \nonumber \\
	& = & A(y_{i-1}-x^*) + x^* - y_{i-1}, \label{eq:link_residue_g_minus_i} \\
	& = & (A-I) \left( \sum_{j=1}^{i-1}\alpha_j x_j + \sum_{j=1}^{i-1} \beta_j y_{j-1} - x^*\right).\nonumber 
\EEA
Since $\sum_{j=1}^{i-1} (\alpha_j+\beta_j) = 1$,
\BEQ
	(A-I) \left( \sum_{j=1}^{i-1}\alpha_j x_j + \sum_{j=1}^{i-1} \beta_j y_{j-1} - x^*\right) = (A-I) \left( \sum_{j=1}^{i-1} \alpha_j (x_j-x^*) + \sum_{j=1}^{i-1} \beta_j (y_{j-1} - x^*)\right).\label{eq:temp1}
\EEQ
We can link $x_j-x^*$ with $y_{j-1}-x^*$ as follow,
\[
	x_j-x^* = A(y_{j-1}-x^*) + x^* - x^* = A(y_{j-1}-x^*).
\]
With this relation, equation \eqref{eq:temp1} simplifies into
\BEAS
    (A-I) \left( \sum_{j=1}^{i-1}\alpha_j (x_j-x^*) + \sum_{j=1}^{i-1} \beta_j (y_{j-1} - x^*)\right) & = & (A-I)  \sum_{j=1}^{i-1}\Big( \left(A\alpha_j +\beta_j\right) (y_{j-1} - x^*)\Big).
\EEAS
In fact, this is a combination of residuals since
\[
    (A-I)(y_j-x^*) = A(y_j-x^*) - y_j = x_{j+1}-y_j = r_{j+1}.
\]
We finally have
\[
    r_{i} = \sum_{j=1}^{i-1} \left(A\alpha_j +\beta_j\right) r_{j-1}.
\]
We assumed by recursion that $r_j = q_j(A)r_1$, where $p_j$ is a polynomial of degree \textit{exactly} $j-1$, and $q_j(1) = 1$. The previous equation is thus equivalent to
\[
	r_{i} = \underbrace{\sum_{j=1}^{i-1} \Big(\alpha_{j} A q_j(A) + \beta_j q_j(A)\Big)}_{=q_i(A)} r_1.
\]
Let us check if $q_i(1) = 1$. Indeed,
\[
	q_i(1) = \sum_{j=1}^{i-1} \Big(\alpha_{j} q_j(1) + \beta_j q_j(1) \Big) = \sum_{j=1}^{i-1} \Big(\alpha_{j} + \beta_j \Big) = 1.
\]
Now, we check if the degree of the polynomial is indeed equal to $i-1$. We have
\BEAS
	\deg (q_i(x)) & = & \deg\left(\sum_{j=0}^{i-1} (\alpha_j x + \beta_j) q_j(x)\right).
\EEAS
Since by assumption $\deg(q_{j}(x))<\deg(q_{i-1}(x))$ for $j<i-1$,
\[
	\deg (q_i(x)) = \deg\left( (\alpha_{i} x + \beta_{i-1}) q_{i-1}(x)\right).
\]
Because $\alpha_{i} \neq 0$ by assumption,
\[
	\deg (q_i(x)) = \deg\left( \alpha_{i} x q_{i-1}(x)\right) = 1+\deg(q_{i-1}(x)).
\]
Finally, because the degree of $q_{i-1}$ is exactly equal to $i-2$,
\[
	\deg (q_i) = i-1.
\]
We proved by recursion that $\deg(q_{i}) = i-1$ and $q_i(1)=1$, which concludes the proof.
\end{proof}

In the next section, we will see how to control the convergence bound in Theorem~\ref{thm:convergence_rate_online_rna}.

% This section showed that convergence analysis of nonlinear acceleration can be reduced to the study of
% \[
%     \min_{p:\mathcal{P}_k, \, p(1) = 1} \|p(A)\|,
% \]
% In the next section and in the rest of the paper, we will restrict our analysis to the special case where $\| \cdot \|$ stands for the $\ell_2$ norm. %The next section will recall results from \citep{scieur2016regularized}, which assumes that $A$ is a symmetric matrix, with $\|A\|_2 < 1$. In this specific setting, it is possible to show optimal rate of convergence of nonlinear acceleration.

==> nonlinear_acceleration_symmetric.tex <==
Here, we assume $A$ is a symmetric matrix, with $\|A\|< 1-\kappa$, for $\kappa \in ]0,1[$. In many applications, such as optimization, $\kappa$ often refers to the \textit{inverse condition number}. \citep{scieur2016regularized} show that extrapolating fixed-step graident descent using nonlinear acceleration algorithm achieves an optimal rate of convergence in the sense of Nesterov \citep{nesterov2013introductory}.

\begin{proposition}\label{prop:conv_cheby_line}
Assume we have a sequence of pairs $(x_{i},y_{i-1})$ generated by \eqref{eq:iter} where
\[
    0 \preceq A \preceq 1-\kappa \;; \qquad \sum_{j=1}^i (\alpha_j^{(i)}+\beta_j^{(i)}) = 1 \quad \text{and} \quad  \alpha_i^{(i)}\neq 0 \qquad \forall \, i=1 \ldots k.
\]
Then the extrapolation $\sum_{i=1}^k c^*_i y_{i-1}$, where $c^*$ is computed using \eqref{eq:cstar}, follows
\[
    \left\| \sum_{i=1}^k c^*_i y_{i-1}-x^* \right\|_2 \leq \frac{1}{\kappa} \frac{2\xi^{k-1}}{1+\xi^{2{k-1}}} \|r_1\|, \quad \xi = \frac{1-\sqrt{\kappa}}{1+\sqrt{\kappa}}.
\]
\end{proposition}
\begin{proof}
We quickly recall the main arguments of the proof present in \citep{scieur2016regularized}. It mainly consists in upper-bounding the term
\BEQ\label{eq:polynomial_before}
    \min_{p\in \mathcal{P}_k, \, p(1) = 1} \|p(A)\|.
\EEQ
Because $A$ is \textit{symmetric}, it suffices to look at the eigenvalue of $A$ which maximizes the norm,
\BEQ\label{eq:polynomial_after}
    \min_{p\in \mathcal{P}_k, \, p(1) = 1} \max_{\lambda_i(A)} |p(\lambda_i)|.
\EEQ
This problem is complex due to the discrete constraints on $\lambda$. However, the maximum can be relaxed on the continuous segment $[0,1-\kappa]$,
\[
    \min_{p\in \mathcal{P}_k, \, p(1) = 1} \max_{\lambda \in [0,1-\kappa]} |p(\lambda)|.
\]
This has been already studied for example by \citet{golub1961chebyshev}, and the solution is given by a ``Chebyshev-like'' polynomial, written
\[
    T_{\kappa,k-1}(x) = \frac{C_{k-1}(t_\kappa(x))}{C_{k-1}(t_\kappa(1))}, \quad t_\kappa(x) = \frac{2x}{1-\kappa}-1,
\]
where $C_{k-1}(x)$ is the Chebyshev polynomial of degree $k-1$. The exact rate of convergence is obtained by evaluating $T_{\kappa,k-1}(x)$ at its maximum value, $x = 1-\kappa$. Finally, the term $\|(I-A)^{-1}\|_2$ is bounded by $\kappa^{-1}$ given the assumption on $A$.
\end{proof}

The crucial part of the proof is moving from \eqref{eq:polynomial_before} to \eqref{eq:polynomial_after}, i.e. moving from matrix polynomials to scalar polynomials on a line segment. This step only works here because $A$ has an orthonormal eigenvalue decomposition with real eigenvalues, i.e. when $A$ is symmetric. We will now recall Crouzeix's conjecture, which will allow us to study the norm of matrix polynomials for non-symmetric matrices. 



==> online_rna.tex <==

In this section, we develop the online-RNA algorithm, which injects the extrapolated point built by RNA directly inside the algorithm. This means accelerating and restarting the algorithm at each step, thus improving its rate of convergence.

\subsection{Online-RNA Algorithm}

The design of the online-RNA algorithm is straightforward. Since the extrapolation is a linear combination of previous iterates, it fits exactly in the template for $y_i$ in method~\eqref{eq:iter} of Section~\ref{s:nacc}, so any algorithm $g(x)$ can be accelerated online as follows,
\BEQ
    \begin{cases}
    x_{i} & = g(y_{i-1})\\
    y_{i} & = \textbf{RNA}(\{(x_j,y_{j-1})\}_{j=1\ldots i},\lambda)
    \end{cases} \label{eq:algo_rna}
\EEQ
where the second step corresponds to the application of Algorithm \eqref{algo:block-rna} using the sequence of $x_j$ and $y_{j-1}$ generated so far. The only restriction, regarding Theorem \ref{thm:convergence_rate_online_rna}, is that the coefficient associated to $x_i$ which should not be zero. This is very unlikely and can be easily fixed by using another value for $\lambda$. Assuming this condition holds, the algorithm has an optimal rate of convergence on quadratic problems.

However, the complexity grows quadratically with $k$, the iteration counter, because this is also the length of sequences $\{x_i\}$ and $\{y_{i-1}\}$. In practice, it is better to use a fixed window where $k$ is bounded. This strategy is similar to the limited version of BFGS, where a fixed number of gradients is stored in memory \citep{boyd2004convex}.


\subsection{Accelerating Algorithms with Momentum Terms}

The main limitation with the online version of RNA is the acceleration of already-accelerated algorithm. Usually, such methods already present an inner linear combination of previous iterates, for example Nesterov's algorithm \citep{nesterov2013introductory}. Combining the online-RNA and already existing linear combination is not that straightforward. A naive, but innefficient way to combine both approaches consists in computing sequentially the extrapolation with RNA then apply the linear combination (or vice-versa), i.e.
\BEQ
    \begin{cases}
        z_{i} & = g(y_{i-1})\\
        x_{i} & = \textbf{RNA}(\{(z_i,y_i)\},\lambda)\\
        y_{i} & = \sum_{j=1}^{i} \left(\alpha_j^{(i)} x_j  + \beta_j^{(i)} y_{j-1}\right)
    \end{cases}. \label{eq:bad_rna}
\EEQ
In fact, the combination of the second and third step is meaningless. At the end, we still end with a linear combination of previous iterates. On one hand, it deteriorates the RNA solution, so it does not correspond to the optimal solution \eqref{eq:cstar}. On the other hand, it does not correspond to the original linear combination, thus potentially voiding theoretical convergence guarantees.

However, some of these methods are designed in a way that the point $x_i$ has to satisfy a ``sufficient descent condition'', satisfied when $x_{i} = g(y_{i-1})$. For example, Nesterov's accelerated gradient can be written
\[
\begin{cases}
    x_{i} & \mbox{such that } f(x_{i}) \leq f(x_{i-1}) -\frac{1}{2L}\|\nabla f(x_{i-1})\|^2_2\\
    y_{i} & = (1+\beta) x_{i} -\beta x_{i-1}
\end{cases}
\]
In this case, the sufficient descent condition is satisfied when $g(x)$ is a gradient step with step length $\frac{1}{L}$. The linear combination in this algorithm ensures a better convergence rate than gradient method, which is not true anymore when using the (bad) strategy described in \eqref{eq:bad_rna}.

In this section, we accelerate methods with momentum that can be written as
\BEQ \label{eq:iter_condition}
    \begin{cases}
        x_{i} &  \mbox{such that } h(x_i,\{(x_{j},y_{j-1})\}_{j=1,\ldots,(i-1)}) \leq 0\\
        y_{i} & = \sum_{j=1}^{i} \left(\alpha_j^{(i)} x_j  + \beta_j^{(i)} y_{j-1}\right)
    \end{cases}
\EEQ
where $h$ can be assimilated, for example, to a sufficient descent condition. Usually, the step in $y_i$ has been designed to ensure a theoretical convergence rate, usually better than applying the simple fixed-point iteration $x_{i} = g(x_{i-1})$. However, the application of online RNA will break this theoretical guarantee. The following algorithm is a slight modification to online RNA, which checks if we can use the extrapolation step while ensuring the theoretical rate of convergence.

 
\begin{algorithm}[h!t]
	\begin{algorithmic}
		\REQUIRE Sequences of $k$ pairs $(x_j,y_{j-1})$ generated by \eqref{eq:iter_condition}, regularization parameter $\lambda$.
		\STATE Compute extrapolation $ x_{\text{extr}} = \textbf{RNA}(\{(x_j,y_{j-1}\},\lambda)$.
		\STATE Compute the conditional point $z_k$, written
		\[
		    z_k = \frac{1}{\alpha_k^{(k)}} \left(x_{\text{extr}} -\sum_{j=1}^{k-1} \alpha_j^{(k)} x_j - \sum_{j=1}^{k} \beta_j^{(k)} y_j\right).
		\]
		\IF{the condition $h(z_k,\{(x_{j},y_{j-1})\}_{j=1,\ldots,(k-1)}) \leq 0$ is satisfied}
        \STATE Use \textbf{RNA} algorithm, $y_k = x_{\text{extr}}$.
        \ELSE
        \STATE Use the original combination, $y_{k} = \sum_{j=1}^{k} \left(\alpha_j^{(k)} x_j  + \beta_j^{(k)} y_{j-1}\right)$.
        \ENDIF
		\STATE 
	\end{algorithmic}
	\caption{Regularized Nonlinear Acceleration for Momentum-based Algorithms}
	\label{algo:momentum-rna}
\end{algorithm}

This method preserves the rate of convergence of the original algorithm, as shown in the following proposition.

\begin{proposition}
Assume we have a proven rate of convergence for $y_i$ when it follows \eqref{eq:iter_condition}. In addition, assume the condition $h(x_i,\{(x_{j},y_{j-1})\}_{j=1,\ldots,(i-1)}) \leq 0$ is satisfied when $x_i = g(y_{i-1})$. Then the sequence generated by Algorithm \ref{algo:momentum-rna} also has the same rate of convergence.
\end{proposition}
\begin{proof}
Indeed, when $z_i$ does not satisfy $h(z_i,\{(x_{j},y_{j-1})\}_{j=1,\ldots,(i-1)}) \leq 0$, then one step of Algorithm \ref{algo:momentum-rna} corresponds exactly to one step of \eqref{eq:iter_condition}. When $z_i$ satisfy the condition, then $y_i$ in \eqref{eq:iter_condition} becomes
\[
    y_{i} = \alpha_i^{(i)}z_i + \sum_{j=1}^{i-1} \alpha_j^{(i)} x_j  + \sum_{j=1}^{i} \beta_j^{(i)} y_{j-1}.
\]
Replacing $z_i$ by its expression gives
\[
    y_i = \sum_{j=1}^i c_j^* x_j,
\]
which preserves the rate of convergence since $z_i$ satisfy the condition.
\end{proof}

In fact, we can see Algorithm \ref{algo:momentum-rna} to be a `smart' line-search technique, since it has the same complexity than a backtracking line search (the function is evaluated two times per iteration). The algorithm is particularly simple when using Nesterov's method because it has only two parameters in the linear combination. The acceleration scheme makes accelerated gradient adaptive to both smoothness and strong convexity constant, while keeping the optimal rate of convergence. We illustrate the explicit acceleration of Nesterov's method in Algorithm \ref{algo:nesterov-rna}. It achieves the optimal $1-\sqrt{\frac{\mu}{L}}$ rate of convergence on smooth and strongly convex functions, and usually performs much better than Nesterov's method. However, we will see in the numerical experiment below that its numerical performance is often worse than simply accelerating gradient descent with the online-RNA scheme, so preserving the optimal theoretical convergence bound has a nontrivial numerical cost here.

\begin{algorithm}[h!t]
	\begin{algorithmic}
	    \REQUIRE Smoothness parameter $L$, strong convexity constant $\mu$, starting point $x_0 = y_0$.
	    \STATE Compute $\beta = \frac{\sqrt{L}-\sqrt{\mu}}{\sqrt{L}+\sqrt{\mu}}$.
		\FOR{$i=1$ to $k$}
    		\STATE Perform a gradient step $x_{i} = y_{i-1}-\frac{1}{L} \nabla f(y_{i-1})$.
    		\STATE Compute the extrapolation $x_{\text{extr}} = \textbf{RNA}(\{x_j,y_{j-1}\},\lambda)$
    		\STATE Compute the conditional point
    		\[ 
    		    z_i = \frac{1}{1+\beta}\left( x_{\text{extr}} + \beta x_{i-1} \right)
    		\]
    		\IF{the descent condition $f(z_i) \leq f(y_i) - \frac{1}{2L} \|\nabla f(y_i)\|_2^2$ is satisfied}
    		    \STATE Use the extrapolation $y_{i} = x_{\text{extr}}$
    		\ELSE
    		    \STATE Use the original combination $y_{i} = (1+\beta) x_i - \beta x_{i-1}$
    		\ENDIF
        \ENDFOR
	\end{algorithmic}
	\caption{Adaptive Optimal First Order Method for Smooth and Strongly Convex Functions}
	\label{algo:nesterov-rna}
\end{algorithm}


==> tmp-pdfcrop-54412.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{6D732D6175746F70702E706466}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{4}
\page 1 [596 598 818 753]
\page 2 [596 597 818 772]
\page 3 [597 597 785 744]
\page 4 [597 597 785 748]
\page 5 [597 597 818 770]
\page 6 [597 597 818 770]
\page 7 [598 597 818 766]
\page 8 [598 597 818 766]
\page 9 [598 599 815 760]
\page 10 [598 599 815 764]
\page 11 [596 595 817 764]
\page 12 [596 595 817 764]

